Optimized Memory System Architecture for VESA VDC-M Decoder with Multi-Slice Support

Video compression plays a pivotal role in managing and transmitting large-scale display data, particularly given the growing demand for higher resolutions and improved video quality. This paper proposes an optimized memory system architecture for Video Electronics Standards Association (VESA) Display Compression-M (VDC-M) decoder, characterized by its substantial on-chip buffer requirements. We design and analyze three architectures categorized by optimization levels and management complexity. Our strategy focuses on enhancing line buffer access scheduling and minimizing reconstruction buffer, targeting prediction and multi-slice operation that are the major resource consumers in the decoder. By adjusting line delay and segmenting SRAM bank alongside reconstructed block forwarding, we achieve a 33.3% size reduction in the line buffer and 77.3% in the reconstruction buffer compared to Baseline VDC-M decoder. Synthesized using a 28 nm CMOS process, the proposed architecture achieves a 31.5% reduction in gate count of the decoder backend hardware, supporting real-time performance with up to 96.45 fps for 4K UHD resolution at 200 MHz operating frequency and a throughput of 4 pixels per cycle.

==> Table1.tex <==
\begin{table}[t]
\caption{Hardware Complexity Comparison between the Proposed DBE Architectures}
\label{tab: Synthesis Results}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{C{4.3cm} | C{2cm} | C{2cm} | C{2cm}}\hline\hline
                                                                           & \textbf{Baseline} & \textbf{Type 1} & \textbf{Type 2} \\\hline\hline
\begin{tabular}[c]{@{}c@{}}Gate Count\\(Including F/F Buffer)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}603,525\\(1,656 B)\end{tabular} &
\begin{tabular}[c]{@{}c@{}}574,072\\(1,400 B)\end{tabular} & 
\begin{tabular}[c]{@{}c@{}}401,850\\(376 B)\end{tabular} \\\hline
\begin{tabular}[c]{@{}c@{}}SRAM Size {[}KB{]}\\(\# of Bank x Bank Size)\end{tabular}                                                     
&3x15.36  
& 2x15.36  
& 4x7.68 \\\hline\hline
\end{tabular}}
\end{table}

==> Table2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{Comparison with DSC Decoders}
\begin{threeparttable}
\label{tab: Synthesis Results}
\resizebox{\columnwidth}{!}{
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{cc|c|c|c|c|c}
\hline\hline
\multicolumn{2}{c|}{}                                                                                                                                                          
& \begin{tabular}[c]{@{}c@{}}MWSCAS'18\\ {[}10{]}\end{tabular}               
& \begin{tabular}[c]{@{}c@{}}T-CE'19\\ {[}11{]}\end{tabular}                                
& \begin{tabular}[c]{@{}c@{}}TCAS-II'21\\ {[}12{]}\end{tabular}              
& \begin{tabular}[c]{@{}c@{}}VLSI-SoC'22\\ {[}13{]}\end{tabular} 
& \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}This Work\\ (Type 2)\end{tabular}}}                 
\\ \hline\hline

\multicolumn{2}{c|}{Standard}                                                                                                                                                  
& DSC v1.2a                                                                  
& DSC v1.1                                                                                  
& DSC v1.2a                                                                  
& DSC v1.2a                                                      
& \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} VDC-M v1.2}                                                                   
\\ \hline

\multicolumn{2}{c|}{Feature}                                                                                                                                                   
& \begin{tabular}[c]{@{}c@{}}Slice\\Interleaving\end{tabular}               
& \begin{tabular}[c]{@{}c@{}}Line Buffer\\Optimization\end{tabular}                        
& \begin{tabular}[c]{@{}c@{}}Many Core\\Processor\\Array\end{tabular}      
& \begin{tabular}[c]{@{}c@{}}FPGA\\Implementation\end{tabular}  
& \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}Line \& Rec.\\Buffer\\Optimization\end{tabular}}
\\ \hline

\multicolumn{2}{c|}{\# of Slices}                                                                                                                                              
& 4                                                                          
& 1                                                                                        
& 4                                                                          
& 1                                                              
& \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} \textbf{4}}                                                                            
\\ \hline

\multicolumn{2}{c|}{Resolution}                                                                                                                                             
& 7680x4320                                              
& 2560x1440                                           
& 1920x1080                                          
& 3840x2160                                        
& \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 3840x2160}         
\\ \hline

\multicolumn{2}{c|}{Technology}                                
& 28 nm                                                       
& 65 nm                                                      
& 32 nm                                                 
& \begin{tabular}[c]{@{}c@{}}Kintex\tnote{1}\\Ultrascale+\end{tabular}  
& \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 28 nm}                            
\\ \hline

\multicolumn{2}{c|}{Operating Frequency}                             
& 1.04 GHz                                                  
& 82 MHz                                                       
& 1.75 GHz                                              
& 262 MHz                                                
& \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} 200 MHz}    
\\ \hline

\multicolumn{2}{c|}{}                                    
& 3.11 G                                                
& 246 M                                                    
& 99.3 M                                   
& 262 M                                          
& \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} \textbf{800 M}}   
\\

\multicolumn{2}{c|}{}                               
& 6.22 G                                              
&                                                    
& 198.27 M                                            
& 524 M                                                
& \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} \textbf{800 M}}     
\\

\multicolumn{2}{c|}{\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Decoding\\Throughput\tnote{2}\\{[}Pixels/s{]}\end{tabular}}}     
& 6.22 G                                                         
&                       
& 296.27 M                                                       
& 524 M                                                
& \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} }           
\\ \hline

\multicolumn{1}{c|}{}                                            
&                                                                  
&                                                                 
&                                                                
&                                                               
&                                                          
& \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} }          
\\

\multicolumn{1}{c|}{}                                               
& \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Line\\Buffer\end{tabular}} 
& \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}30.9 KB\\(SRAM)\end{tabular}} 
& \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}9.6 KB\textsuperscript{†} (SRAM)\\48.75 B\textsuperscript{†}(F/F)\end{tabular}} 
&                                                                            
& \multirow{-2}{*}{Not Provided}                                 
& \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}30.72 KB\\(SRAM)\end{tabular}}}           
\\ \cline{2-4} \cline{6-7} 

\multicolumn{1}{c|}{\multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}Memory\tnote{3}\\Requirement\end{tabular}}} 
& \begin{tabular}[c]{@{}c@{}}Rec. / ICH\\Buffer\end{tabular}             
& Not Provided                                                             
& Not Provided                                                              
& \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}256 KB\tnote{‡}\\ (SRAM)\end{tabular}} 
& \begin{tabular}[c]{@{}c@{}}120 B\tnote{†}\\(F/F)\end{tabular}      
& \cellcolor[HTML]{EFEFEF}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}376 B\\(F/F)\end{tabular}}}             
\\ \hline\hline

\end{tabular}}
\begin{tablenotes}
    \item[ ] \tiny{ }
    \item[†] \scriptsize{A color bit depth of 10 bpc is assumed.}
    \item[‡] \scriptsize{Estimated value using data from Bohnenstiehl [14]}
    \item[1] \scriptsize{The design is implemented on a Kintex Ultrascale+ FPGA device.}
    \item[2] \scriptsize{Decoding throughput of 4:4:4, 4:2:2, and 4:2:0 pixel formats are reported in the\\top, middle, bottom of the columns, respectively.}
    \item[3] \scriptsize{Memory requirement for a color bit depth of 10 bpc among designs provided in\\the paper.}
\end{tablenotes}
\end{threeparttable}
\end{table}






==> Table3.tex <==
\begin{table}[]
\caption{Comparison with DSC Decoders}
\end{table}
